Nonparametric Maximum Likelihood Estimation for Mixtures of Logistic Regressions

Mixtures of logistic regressions provide a flexible framework for modeling binary responses, extending standard logistic regression to accommodate unobserved heterogeneity while retaining an interpretable regression structure. In this paper, we study such models with an unspecified mixing distribution. We analyze a sieve nonparametric maximum likelihood estimator (NPMLE) and derive nonasymptotic bounds on the estimation error of the resulting mixture regression function under both fixed and random designs. Our results reveal an explicit tradeoff between statistical estimation error and the approximation error induced by the sieve radius, from which we derive convergence rates under several tail conditions on the mixing distribution. For computation, we propose a finite-particle algorithm that approximates the sieve NPMLE by optimizing the locations and weights of a finitely supported mixing distribution. The method offers numerical advantages over existing algorithms and comes with rigorous convergence guarantees. For any fixed dataset, we establish global convergence of the likelihood to the restricted NPMLE value when the number of particles exceeds a finite threshold. When the true mixing distribution is finitely supported, we further establish uniform global convergence guarantees and derive error bounds that separate algorithmic and statistical errors. Our analysis also yields a denoising bound for the mixing distribution and an identifiability result that complements existing results in the literature.

==> manuscript/preamble.tex <==
\usepackage{amsthm,amsmath,amsfonts,amssymb,mathtools,mathrsfs,bm}
\usepackage{multirow,graphicx,booktabs,url,xcolor,enumitem,algorithm}

\RequirePackage[authoryear]{natbib}
\usepackage[colorlinks=true,
linkcolor=blue,
urlcolor=blue,
citecolor=blue]{hyperref}
\usepackage{longtable,array}
\usepackage[capitalize]{cleveref}
\usepackage{tabularx,threeparttable,needspace}
\usepackage{simulation_labels}
\usepackage{xb_preamble}
\usepackage{algpseudocode}

\makeatletter
\@ifclassloaded{imsart}{
\def\nocontentsline{
  \let\@@addcontentsline\addcontentsline
  \def\addcontentsline##1##2##3{\let\addcontentsline\@@addcontentsline}
}
\startlocaldefs
}{}
\makeatother

\numberwithin{equation}{section}
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\makeatletter
\@ifclassloaded{imsart}{\theoremstyle{definition}}{}
\makeatother
\newtheorem{assumption}{Assumption}
\newtheorem{fact}{Fact}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{theorem}{Theorem}{Theorems}

\crefname{appendix}{Appendix}{Appendices} 

\newtheorem{innercustomgeneric}{\customgenericname}
\providecommand{\customgenericname}{}
\newcommand{\newcustomtheorem}[2]{\newenvironment{#1}[1] {\renewcommand\customgenericname{#2}\renewcommand\theinnercustomgeneric{##1}\innercustomgeneric
  }{\endinnercustomgeneric}
}

\newcustomtheorem{customass}{Assumption}
\theoremstyle{definition}
\newtheorem{remark}{Remark}

\def\Bern{{\rm Bern}}
\def\app{{\textsf{app}}}
\def\est{{\textsf{est}}}
\def\mfa{{\mathfrak a}}
\def\bd{{\bm b}}
\def\bdelta{{\bm \delta}}

\makeatletter
\@ifclassloaded{imsart}{\endlocaldefs}{}
\makeatother

